An Instance-Based Approach to the Trace Reconstruction Problem

In the trace reconstruction problem, one observes the output of passing a binary string $s \in \{0,1\}^n$ through a deletion channel $T$ times and wishes to recover $s$ from the resulting $T$ "traces." Most of the literature has focused on characterizing the hardness of this problem in terms of the number of traces $T$ needed for perfect reconstruction either in the worst case or in the average case (over input sequences $s$). In this paper, we propose an alternative, instance-based approach to the problem. We define the "Levenshtein difficulty" of a problem instance $(s,T)$ as the probability that the resulting traces do not provide enough information for correct recovery with full certainty. One can then try to characterize, for a specific $s$, how $T$ needs to scale in order for the Levenshtein difficulty to go to zero, and seek reconstruction algorithms that match this scaling for each $s$. We derive a lower bound on the Levenshtein difficulty, and prove that $T$ needs to scale exponentially fast in $n$ for the Levenshtein difficulty to approach zero for a very broad class of strings. For a class of binary strings with alternating long runs, we design an algorithm whose probability of reconstruction error approaches zero whenever the Levenshtein difficulty approaches zero. For this class, we also prove that the error probability of this algorithm decays to zero at least as fast as the Levenshtein difficulty.

==> introduction02-03.tex <==
\section{Introduction}

In the trace reconstruction problem, there exists a binary source string $s \in \{0, 1\}^n$, and we are given a set $\cT$ of $T$ traces of $s$, where a trace is a subsequence of $s$.  We are then asked to reconstruct $s$ from $\cT$.  This problem been studied by many researchers in computer science, electrical engineering, and mathematics due to its fundamental nature, and applicability to sequence alignment, phylogeny, DNA data storage, and computational biology \cite{Pfevzner, Yaakobi}.

Levenshtein introduced this problem in 2001 as the ``sequence reconstruction problem'' \cite{Lev1, Lev2}, and studied for a worst case source string $s$, how many distinct worst-case traces of a given length are needed so that the only string that the traces could have arisen from is $s$ itself.  
Since both the source string and the set of distinct traces are both worst-case, the number of distinct traces needed is very large.  
\iscomment{not clear how this problem is well defined}
\kmcomment{I tried making it more clear}
In 2004, Batu et al. \cite{Batu} studied the problem in the case where each bit in $s$ is deleted independently with probability $p$ to form each trace, referring to it as ``trace reconstruction.''  The authors derived an algorithm to reconstruct any length $n$ string $s$ with probability approaching one as $n$ increases using an exponential number of traces in $n$, and derived a lower bound on the number of traces required by any algorithm to reconstruct $s$ with probability approaching one as $n$ increases. This is referred to as the ``worst-case trace reconstruction problem.''  The authors also showed that if $s$ is chosen uniformly at random, much fewer traces can be used to reconstruct $s$ with probability approaching one.  This is referred to as the ``average-case trace reconstruction problem.''   Many developments have been made for both the worst case and the average case versions of the problem.  
For the worst case version of the problem, which is more similar to our problem, a large gap still exists between upper and lower bounds on the number of traces required.  Currently, the best lower bound, due to Chase, is $\tilde{\Omega}(n^{3/2})$~\cite{Chase2}, while the best upper bound, due to Chase, is $\exp(\tilde{O}(n^{1/5}))$ \cite{Chase}.

In this paper, we consider a hybrid between the Levenshtein's sequence reconstruction problem and the worst case trace reconstruction problem.  A set $\cT$ of  $T$ traces  {\it unambiguously reconstructs} $s \in \{0, 1\}^n$ if the only length $n$ binary string that $\cT$ could have arisen from is $s$. We seek necessary and sufficient conditions on the set of traces to unambigiously reconstruct $s$, and study the probability of these conditions holding when the traces are randomly generated with fixed deletion probability $p$. 
This problem setup is motivated by  situations where we want to know that $s$ has been reconstructed correctly with certainty, and is fundamental from an information theory perspective.
Our setup is similar to Levenshtein's sequence reconstruction problem in that we study unambiguous reconstruction, but is different because we study when an arbitrary set of traces unambiguously reconstructs $s$, as opposed to only studying when the worst case set of distinct traces of a given length unambiguously reconstructs $s$.  In our statistical analysis, we consider the same trace generation model used in the worst-case trace reconstruction problem where each trace is generated by deleting each bit in $s$ independently with probability $p$.  However, our problem is different in that we focus on unambiguous reconstruction whereas worst-case trace reconstruction focuses on reconstruction with high probability.

To initiate the study of this problem, we derive several necessary conditions on $s$ and $\cT$ for unambiguous reconstitution.  We then derive a sufficient condition for unambiguous reconstruction that yields an efficient algorithm, and show that for a certain class $\cS$ of source strings $s \in \{0,1\}^n$, the probability of the sufficient condition not holding in the statistical model approaches the probability of the necessary conditions not holding for $T = \exp(cn)$ traces as $n$ increases when $c > c^*$ where $c^*$ is a positive constant that depends of the source string.  This shows that the efficient  algorithm we design based off the sufficient condition is information-optimal for $\cS$ and this choice of $T$, motivating the discovery of new information-optimal algorithms for this problem. 


==> larger_than_exp_T.tex <==
	\section{Analysis for larger growth rates of $T$}
	\subsection{Analysis of $\Pr(\bar{E}_1)$ for larger growth rates of $T$}
	
	Suppose that $s$ has $M$ runs, and the length of the $i$th run in $s$ is equal to $\ell_i m$.
	Suppose the number of traces is $T = f(m)$ where $f(m) = \omega(\exp(cm))$ for all positive constants $c$.
	For ease of presentation, let $q_i = \ell_i$ and $u_i = \ell_i f^{-1}(T)$. Let $X \sim \text{Bin}(T, \; \prod_{i=1}^M (1-p^{u_i}))$ be the binomial random variable with $T$ trials and probability parameter $p_X = \prod_{i=1}^M (1-p^{u_i})$.
	According to the formula in the previous section, we have 
	\begin{align}
		& \Pr(\bar{E}_1) = 1 - \prod_{i = 1}^M (1 - (1 - (1-p)^{q_i f^{-1}(T) })^T ) \nonumber 
		\\ & = \sum_{y = 1}^M \; \sum_{K \subseteq [M] : \; |K| = y} (-1)^{y+1} \prod_{i \in K}  (1 - (1-p)^{q_i f^{-1}(T)})^T.
	\end{align}
    Thus, we have to find the asymptotic behavior of $\left(\prod_{i \in K} (1 - (1-p)^{q_i f^{-1}(T)})\right)^T$ for general $K \subseteq [M].$	We have that 
	\begin{align}
		&  \left(\prod_{i \in K} (1 - (1-p)^{q_i f^{-1}(T)})\right)^T \nonumber
		\\ & =  \exp \left( \log \left(  \left(\prod_{i \in K} (1 - (1-p)^{q_i f^{-1}(T)})\right)^T \right) \right) \nonumber
		\\ & = \exp \left( T \log   \left(\prod_{i \in K} (1 - (1-p)^{q_i f^{-1}(T)})\right) \right) \nonumber
		\\ & = \exp \left(  T \log   \left(\prod_{i \in K} (1 - (1-p)^{q_i f^{-1}(T)})\right) \right) \nonumber
		\\ & = \exp \left(  T \sum_{i \in K} \log \left(1 - (1-p)^{q_i f^{-1}(T)}\right) \right) \nonumber
		\\ & \sim \exp \left(   T \sum_{i \in K}   -(1-p)^{q_i f^{-1}(T)} \right) \nonumber
		\\ & = \prod_{i \in K} \exp \left( -  T (1-p)^{q_i f^{-1}(T)}\right).
	\end{align}
	then all the terms in the expanded form of $P(\bar{E}_1)$ approach zero as $T$ increases and we have that
	\begin{align}
		\Pr(\bar{E}_1) \sim \sum_{i \in [M]} \exp \left( -  T (1-p)^{q_{i} f^{-1}(T)}\right).
	\end{align}  


	\subsection{Analysis of $\Pr(\bar{E}_2)$ for larger growth rates of $T$}
	
	Suppose that $s$ has $M$ runs, and the length of the $i$th run in $s$ is equal to $\ell_i m$.
	Suppose the number of traces is $T = f(m)$ where $f(m) = \omega(\exp(cm))$ for all positive constants $c$.
	For ease of presentation, let $q_i = \ell_i$ and $u_i = \ell_i f^{-1}(T)$. Let $X \sim \text{Bin}(T, \; \prod_{i=1}^M (1-p^{u_i}))$ be the binomial random variable with $T$ trials and probability parameter $p_X = \prod_{i=1}^M (1-p^{u_i})$. From the previous section, we have that
	\begin{align}
		& \Pr(\bar{E}_2) = 1 - \E \left[ \prod_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{u_i}}{1 - p^{u_i}} \right)^{X}\right) \right] \nonumber
		\\ & = \sum_{y = 1}^M \; \sum_{K \subseteq [M] : \; |K| = y} (-1)^{y+1} \nonumber 
		\\ & \quad \times \left( 1 - p_X + p_X \prod_{i \in K}\left(1 - \frac{(1-p)^{u_i}}{1 - p^{u_i}} \right) \right)^T.
	\end{align}
	Thus, we have to find the asymptotic formula for 
	\[  \left( 1 - p_X + p_X \prod_{i \in K}\left(1 - \frac{(1-p)^{u_i}}{1 - p^{u_i}} \right) \right)^T \]
	for general $K \subseteq [M].$  We have that
	\begin{align}
	    & \left( 1 - p_X + p_X \prod_{i \in K}\left(1 - \frac{(1-p)^{u_i}}{1 - p^{u_i}} \right) \right)^T \nonumber
	    \\ & = \exp\left( T\log \left( 1 - p_X + p_X \prod_{i \in K}\left(1 - \frac{(1-p)^{\ell_i f^{-1}(T)}}{1 - p^{\ell_i f^{-1}(T)}} \right) \right) \right) \nonumber
	    \\ & = \exp\left( T\log \left( 1 - p_X\left(1 - \prod_{i \in K}\left(1 - \frac{(1-p)^{\ell_i f^{-1}(T)}}{1 - (1-p)^{\ell_i f^{-1}(T)}} \right) \right) \right) \right) \nonumber
	    \\ & \sim \exp\left( - T  p_X\left(1 - \prod_{i \in K}\left(1 - \frac{(1-p)^{\ell_i f^{-1}(T)}}{1 - (1-p)^{\ell_i f^{-1}(T)}} \right) \right) \right)  \nonumber
	    \\ & = \exp\left( - T  p_X\left( \sum_{y = 1}^{|K|} \; \sum_{S \subseteq K : \; |S| = y} (-1)^{y+1} \prod_{i \in S} \frac{(1-p)^{\ell_i f^{-1}(T)}}{1 - (1-p)^{\ell_i f^{-1}(T)}} \right) \right)  \nonumber
	    \\ & = \prod_{y = 1}^{|K|} \; \prod_{S \subseteq K : \; |S| = y} \exp\left( - T  p_X  (-1)^{y+1} \prod_{i \in S} \frac{(1-p)^{\ell_i f^{-1}(T)}}{1 - (1-p)^{\ell_i f^{-1}(T)}}  \right)  \nonumber
	\end{align}
	Observe that any term for a non-singleton $K = Z$ is little-o of the term for $K = \{z\}$ where $z \in Z$.   Thus, only the terms corresponding to singleton $K$ in $\Pr(\bar{E}_2)$ can matter asymptotically, leaving us with the following asymptotic formula for $\Pr(\bar{E}_2)$:
	\begin{align}
		\sum_{i=1}^M \exp \left( - T  \left( \prod_{k=1}^M (1-p^{q_k f^{-1}(T)}) \right) \left( \frac{(1-p)^{q_i f^{-1}(T)}}{1 - (1-p)^{q_i f^{-1}(T)}}  \right) \right).
	\end{align}
	Observe that 
	\begin{align}
	    & \frac{\Pr(\bar{E}_2)}{\Pr(\bar{E}_1)}  
		\sim \frac{ \sum_{i=1}^M \exp \left( - T  \left( \prod_{k=1}^M (1-p^{q_k f^{-1}(T)}) \right) \left( \frac{(1-p)^{q_i f^{-1}(T)}}{1 - (1-p)^{q_i f^{-1}(T)}}  \right) \right)}{\sum_{i = 1}{M} \exp \left( -  T (1-p)^{q_{i} f^{-1}(T)}\right)}
		\nonumber
% 		\\ & = \exp \bigg(    \left(  1 - \prod_{k \in [M] \backslash \{i^*\}} (1-T^{q_k \log(p)}) \right) 
% 		 \left( T^{1 + \log(1-p) q_{i^*}}  \right) \bigg) \nonumber
% 		\\ & = \exp \Bigg(   \left(   \sum_{y = 1}^{M-1} \; \sum_{S \subseteq [M] \backslash \{i^*\} : \; |S| = y} (-1)^{y+1} \prod_{i \in S} T^{q_i \log(p)} \right) \nonumber
% 		\\ & \quad \times \left( T^{1 + \log(1-p) q_{i^*}}  \right) \Bigg) \nonumber 
% 		\\ & = \exp \Bigg(      \sum_{y = 1}^{M-1} \sum_{S \subseteq [M] \backslash \{i^*\} : \; |S| = y} (-1)^{y+1}  \nonumber
% 		\\ & \quad \times T^{\sum_{i \in S} q_i \log(p) + 1 + \log(1-p) q_{i^*} }  \Bigg) \nonumber 
% 		\\ & \sim 1
	\end{align}


==> polynomial_T_analysis.tex <==
\section{Analysis when $T$ is polynomial in $n$}
	Let where $E_1$ be the event that each run is fully preserved in at least one trace.  	Let $E_2$ be the event that for each run in $s,$ there is at least one trace that has the run fully preserved and has no run fully deleted. We know that
	\begin{align}
		\Pr(E_1) = \Pi_{i = 1}^M (1 - (1 - (1-p)^{\ell_i})^T ).
	\end{align}
	
	Suppose that $s$ has $M$ runs, and the length of the $i$th run in $s$ is equal to $\ell_i m$.
	Suppose the number of traces is $T = cm^b$ where $c$ and $b$ are positive  constants.  For ease of presentation, let $q_i = \ell_i (1/c)^{1/b}$.
    We then have 
	\begin{align}
		& \Pr(\bar{E}_1) = 1 - \Pi_{i = 1}^M (1 - (1 - (1-p)^{q_i T^{1/b} })^T ) 
		\\ & = \sum_{i = 1}^M (1 - (1-p)^{q_i T^{1/b}})^T  - \sum_{i, j} \left((1 - (1-p)^{q_i T^{1/b}}) (1 - (1-p)^{q_j T^{1/b}})\right)^T + \; \dots \; + (-1)^{M+1} \left(\Pi_{i = 1}^M (1 - (1-p)^{q_i T^{1/b}})\right)^T.
	\end{align}
    Thus, we have to find the asymptotic behavior of $\left(\Pi_{i \in K} (1 - (1-p)^{q_i T^{1/b}})\right)^T$ for general $K \subseteq [M].$	We have that 
	\begin{align}
		& = \left(\Pi_{i \in K} (1 - (1-p)^{q_i T^{1/b}})\right)^T 
		\\ & =  \exp \left( \log \left(  \left(\Pi_{i \in K} (1 - (1-p)^{q_i T^{1/b}})\right)^T \right) \right) 
		\\ & = \exp \left( T \log   \left(\Pi_{i \in K} (1 - (1-p)^{q_i T^{1/b}})\right) \right) 
		\\ & = \exp \left(  T \sum_{i \in K} \log \left(1 - (1-p)^{q_i T^{1/b}}\right) \right) 
		\\ & \sim \exp \left(  - T \sum_{i \in K}   (1-p)^{q_i T^{1/b}} \right)
		\\ & =   \prod_{i \in K}\exp \left(  - T   (1-p)^{q_i T^{1/b}} \right)
		\\ & \to 1.
	\end{align}
    Therefore, we have
	\begin{align}
		& \lim_{T \to \infty }\Pr(\bar{E}_1)	 = \sum_{i = 1}^M (-1)^{i+1} \binom{M}{i} = 1.
	\end{align}    
    by the well known formula $\sum_{i=0}^M (-1)^i \binom{M}{i} = 0$.
	This implies that $\lim_{T \to \infty }\Pr(\bar{E}_2) = 1$ as well.

==> references.tex <==
	\begin{thebibliography}{00}
	
	    \bibitem{Lev1}
	    V. Levenshtein. Efficient reconstruction of sequences. IEEE Transactions
        on Information Theory, 47(1):2–22, 2001.

        \bibitem{Lev2}
        V. Levenshtein. Efficient reconstruction of sequences from their
        subsequences or supersequences. Journal of Combinatorial Theory Series
        A, 93(2):310–332, 2001.
		
		\bibitem{Batu}
		T. Batu S. Kannan, S. Khanna, A. McGregor, ``Reconstructing Strings from Random Traces,'' SODA 2004.	    
		\bibitem{Pfevzner}
		V. Bhardwaj, P. Pevzner, C. Rashtchian, Y. Safonova, ``Trace Reconstruction Problems in Computational Biology,''  Arxiv.
		
		\bibitem{Yaakobi}
		O. Sabary, A. Yucovich, G. Shapira, E. Yaakobi, ``Reconstruction Algorithms for DNA-Storage Systems,'' Arxiv.

		\bibitem{Yaakobi2}
		O. Sabary, E. Yaakobi,	A. Yucovich, ``The Error Probability of Maximum-Likelihood
		Decoding over Two Deletion/Insertion Channels,'' ISIT 2020.
		
		\bibitem{Mitzenmacher}
		T. Holenstein, M. Mitzenmacher, R. Panigrahy, U. Wieder, ``Trace reconstruction with constant deletion probability and related
		results,'' SODA 2008.
		
		\bibitem{Peres1}
		Y. Peres, A. Zhai ``Average-case reconstruction for the deletion channel:
		subpolynomially many traces suffice,'' FOCS 2017.
		
		\bibitem{Peres2}
		N. Holden, R. Pemantle, Y. Peres, ``Subpolynomial trace reconstruction for random strings
		and arbitrary deletion probability,'' COLT 2018.
		
		\bibitem{Holenstein}
		T. Holenstein, M. Mitzenmacher, R. Panigrahy, and U. Wieder. ``Trace reconstruction
        with constant deletion probability and related results.'' SODA 2008.
		
		\bibitem{Servedio}
		A. Da, R. O'Donnel, R. Servedio, ``Optimal Mean-Based Algorithms for Trace Reconstruction,'' STOC 2017.

        \bibitem{Chase}	
        Z. Chase, ``Separating Words and Trace Reconstruction,'' STOC 2021.
        
        \bibitem{Chase2}
        Z. Chase. New Lower Bounds for Trace Reconstruction. To appear in Annales
        Institute Henri Poincare: Probability and Statistics, May 2019.
		
		\bibitem{Tse}
		G. Bresler, M. Bresler, D. Tse, ``Optimal assembly for high throughput shotgun
		sequencing,'' BMC Bioinformatics 2013.
		
		\bibitem{Diggavi}
		S. R. Srinivasavaradhan, M. Du, S. Diggavi, C. Fragouli, ``Symbolwise MAP for Multiple Deletion Channels,'' ISIT 2019.
		
		\bibitem{Davies} S. Davies, M. Z. Rácz, B. G. Schiffer and C. Rashtchian, ``Approximate Trace Reconstruction: Algorithms,'' 2021 IEEE International Symposium on Information Theory (ISIT), 2021, pp. 2525-2530.
		
		\bibitem{Lothaire}
		Lothaire, M. (Ed.). (1997). Combinatorics on Words (2nd ed., Cambridge Mathematical Library). Cambridge: Cambridge University Press.
		
        % 		\bibitem{Notredame}
        % 		C. Notredame, ``Recent progress in multiple sequence alignment: a survey,'' Pharmacogenomics, February 2002.
        		
        % 		\bibitem{Warnow}
        % 		T. Warnow, ``Computational Phylogenomics,'' Multiple Sequence Alignment Chapter.

		%	\bibitem{Maddah-Ali}
		%	A. Gholami, M. A. Maddah-Ali, and S. A. Motahari, ``Private shotgun
		%	dna sequencing,'' Proc. of IEEE International Symposium on Information Theory, 2019.
		%	
		%	\bibitem{Maddah-Ali2}
		%	A. Gholami, M. A. Maddah-Ali and S. A. Motahari, ``Private Shotgun DNA Sequencing: A Structured Approach,'' 2019 Iran Workshop on Communication and Information Theory (IWCIT), Tehran, Iran, 2019, pp. 1-6.
		
	\end{thebibliography}

==> tmp.tex <==
	\begin{align}
		& \Pr(\bar{E}_3) = 1 - \sum_{c = 0}^T \nchoosek{T}{c} \left(\Pi_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)^{c}\right) \right) (\Pi_{i=1}^M (1-p^{\ell_i \log(T)}))^{c} (1 - \Pi_{i=1}^M (1-p^{\ell_i \log(T)}))^{T - c}
		\\ & = 1 - \E \left[ \Pi_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)^{X}\right) \right]
		\\ & = 1 - \E \left[ 1 - \sum_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)^{X}  + \sum_{i, j} \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)^{X} \left(1 - \frac{(1-p)^{\ell_j \log(T)}}{1 - p^{\ell_j \log(T)}} \right)^{X} + \; \dots \; + (-1)^M \left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)^{X} \right) \right]
		\\ & =  \sum_{i = 1}^M \E \left[\left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)^{X} \right]  - \sum_{i, j} \E \left[ \left( \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \left(1 - \frac{(1-p)^{\ell_j \log(T)}}{1 - p^{\ell_j \log(T)}} \right) \right)^{X} \right] + \; \dots \; + (-1)^{M+1} \E \left[ \left( \Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)\right)^{X}  \right] 
		\\ & =  \sum_{i = 1}^M \E \left[e^{\log\left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) X} \right]  - \sum_{i, j} \E \left[ e^{\log\left( \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \left(1 - \frac{(1-p)^{\ell_j \log(T)}}{1 - p^{\ell_j \log(T)}} \right) \right) X} \right] + \; \dots \; + (-1)^{M+1} \E \left[ e^{ \log\left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \right) X}  \right] 
		\\ & =  \sum_{i = 1}^M \left(1 - \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) +  \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) e^{\log\left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right)} \right)^T  
		\\ & - \sum_{i, j} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k \log(T)})  +  \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) e^{\log\left( \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \left(1 - \frac{(1-p)^{\ell_j \log(T)}}{1 - p^{\ell_j \log(T)}} \right) \right)} \right)^T   
		\\ & + \; \dots 
		\\ &  + (-1)^{M+1} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k \log(T)})  +  \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) e^{\log\left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \right)} \right)^T 
		\\ & =  \sum_{i = 1}^M \left(1 - \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) +  \Pi_{k=1}^M (1-p^{\ell_k \log(T)})\left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \right)^T  
		\\ & - \sum_{i, j} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k \log(T)})  +  \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) \left( \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \left(1 - \frac{(1-p)^{\ell_j \log(T)}}{1 - p^{\ell_j \log(T)}} \right) \right) \right)^T   
		\\ & + \; \dots 
		\\ &  + (-1)^{M+1} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k \log(T)})  +  \Pi_{k=1}^M (1-p^{\ell_k \log(T)}) \left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i \log(T)}}{1 - p^{\ell_i \log(T)}} \right) \right) \right)^T 
	\end{align}


==> tmp2.tex <==
	\begin{align}
		& \Pr(\bar{E}_3) = 1 - \sum_{c = 0}^T \nchoosek{T}{c} \left(\Pi_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)^{c}\right) \right) (\Pi_{i=1}^M (1-p^{r_i}))^{c} (1 - \Pi_{i=1}^M (1-p^{r_i}))^{T - c}
		\\ & = 1 - \E \left[ \Pi_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)^{X}\right) \right]
		\\ & = 1 - \E \left[ 1 - \sum_{i = 1}^M \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)^{X}  + \sum_{i, j} \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)^{X} \left(1 - \frac{(1-p)^{r_j}}{1 - p^{r_j}} \right)^{X} + \; \dots \; + (-1)^M \left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)^{X} \right) \right]
		\\ & =  \sum_{i = 1}^M \E \left[\left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)^{X} \right]  - \sum_{i, j} \E \left[ \left( \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \left(1 - \frac{(1-p)^{r_j}}{1 - p^{r_j}} \right) \right)^{X} \right] + \; \dots \; + (-1)^{M+1} \E \left[ \left( \Pi_{i = 1}^M \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)\right)^{X}  \right] 
		\\ & =  \sum_{i = 1}^M \E \left[e^{\log\left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) X} \right]  - \sum_{i, j} \E \left[ e^{\log\left( \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \left(1 - \frac{(1-p)^{r_j}}{1 - p^{r_j}} \right) \right) X} \right] + \; \dots \; + (-1)^{M+1} \E \left[ e^{ \log\left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \right) X}  \right] 
		\\ & =  \sum_{i = 1}^M \left(1 - \Pi_{k=1}^M (1-p^{r_k}) +  \Pi_{k=1}^M (1-p^{r_k}) e^{\log\left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right)} \right)^T  
		\\ & - \sum_{i, j} \left(1 - \Pi_{k=1}^M (1-p^{r_k})  +  \Pi_{k=1}^M (1-p^{r_k}) e^{\log\left( \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \left(1 - \frac{(1-p)^{r_j}}{1 - p^{r_j}} \right) \right)} \right)^T   
		\\ & + \; \dots 
		\\ &  + (-1)^{M+1} \left(1 - \Pi_{k=1}^M (1-p^{r_k})  +  \Pi_{k=1}^M (1-p^{r_k}) e^{\log\left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \right)} \right)^T 
		\\ & =  \sum_{i = 1}^M \left(1 - \Pi_{k=1}^M (1-p^{r_k}) +  \Pi_{k=1}^M (1-p^{r_k})\left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \right)^T  
		\\ & - \sum_{i, j} \left(1 - \Pi_{k=1}^M (1-p^{r_k})  +  \Pi_{k=1}^M (1-p^{r_k}) \left( \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \left(1 - \frac{(1-p)^{r_j}}{1 - p^{r_j}} \right) \right) \right)^T   
		\\ & + \; \dots 
		\\ &  + (-1)^{M+1} \left(1 - \Pi_{k=1}^M (1-p^{r_k})  +  \Pi_{k=1}^M (1-p^{r_k}) \left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{r_i}}{1 - p^{r_i}} \right) \right) \right)^T 
	\end{align}



	
	
	\begin{align}
		& \Pr(\bar{E}_3) = 1 - \sum_{c = 0}^T \nchoosek{T}{c} \left(\Pi_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)^{c}\right) \right) (\Pi_{i=1}^M (1-p^{\ell_i}))^{c} (1 - \Pi_{i=1}^M (1-p^{\ell_i}))^{T - c}
		\\ & = 1 - \E \left[ \Pi_{i=1}^M \left(1 - \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)^{X}\right) \right]
		\\ & = 1 - \E \left[ 1 - \sum_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)^{X}  + \sum_{i, j} \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)^{X} \left(1 - \frac{(1-p)^{\ell_j}}{1 - p^{\ell_j}} \right)^{X} + \; \dots \; + (-1)^M \left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)^{X} \right) \right]
		\\ & =  \sum_{i = 1}^M \E \left[\left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)^{X} \right]  - \sum_{i, j} \E \left[ \left( \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \left(1 - \frac{(1-p)^{\ell_j}}{1 - p^{\ell_j}} \right) \right)^{X} \right] + \; \dots \; + (-1)^{M+1} \E \left[ \left( \Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)\right)^{X}  \right] 
		\\ & =  \sum_{i = 1}^M \E \left[e^{\log\left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) X} \right]  - \sum_{i, j} \E \left[ e^{\log\left( \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \left(1 - \frac{(1-p)^{\ell_j}}{1 - p^{\ell_j}} \right) \right) X} \right] + \; \dots \; + (-1)^{M+1} \E \left[ e^{ \log\left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \right) X}  \right] 
		\\ & =  \sum_{i = 1}^M \left(1 - \Pi_{k=1}^M (1-p^{\ell_k}) +  \Pi_{k=1}^M (1-p^{\ell_k}) e^{\log\left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right)} \right)^T  
		\\ & - \sum_{i, j} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k})  +  \Pi_{k=1}^M (1-p^{\ell_k}) e^{\log\left( \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \left(1 - \frac{(1-p)^{\ell_j}}{1 - p^{\ell_j}} \right) \right)} \right)^T   
		\\ & + \; \dots 
		\\ &  + (-1)^{M+1} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k})  +  \Pi_{k=1}^M (1-p^{\ell_k}) e^{\log\left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \right)} \right)^T 
		\\ & =  \sum_{i = 1}^M \left(1 - \Pi_{k=1}^M (1-p^{\ell_k}) +  \Pi_{k=1}^M (1-p^{\ell_k})\left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \right)^T  
		\\ & - \sum_{i, j} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k})  +  \Pi_{k=1}^M (1-p^{\ell_k}) \left( \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \left(1 - \frac{(1-p)^{\ell_j}}{1 - p^{\ell_j}} \right) \right) \right)^T   
		\\ & + \; \dots 
		\\ &  + (-1)^{M+1} \left(1 - \Pi_{k=1}^M (1-p^{\ell_k})  +  \Pi_{k=1}^M (1-p^{\ell_k}) \left(\Pi_{i = 1}^M \left(1 - \frac{(1-p)^{\ell_i}}{1 - p^{\ell_i}} \right) \right) \right)^T 
	\end{align}
	
